Resource Efficiency vs Performance Isolation Tradeoff in Network Slicing

We consider the tradeoff between resource efficiency and performance isolation that emerges when multiplexing the resource demands of Network Slices (NSs). On the one hand, multiplexing allows the use of idle resources, which increases resource efficiency. On the other hand, the performance of each NS becomes susceptible to traffic surges in other NSs, which degrades performance isolation. The analysis of this tradeoff enables network operators to determine the effect of performance isolation on the operating cost of each NS. To study the tradeoff, we solve an optimization problem where we find the multiplexing policy that requires the least provisioned resources to honor the Service Level Agreements (SLAs) of all NSs. The SLA of each NS i states that its resource demand should be met for $P^H_i$ fraction of time, and for $P^L_i \leq P^H_i$ fraction of time, it should be met regardless of the demands of other NSs. For resource demands that follow ergodic Markov chains, we show that the well-known Max-Weight scheduler is an optimal multiplexing policy. Since the Max-Weight scheduler does not require any knowledge of the statistics of the resource demands, we also propose its use in non-markovian settings. For resource demands obtained in the LTE module of ns-3, we show that the Max-Weight scheduler reduces the provisioned bandwidth by 36.2% when no performance isolation is required. Lastly, for these non-markovian resource demands, the Max-Weight scheduler maintains its optimality since it requires as much provisioned bandwidth as the best non-causal scheduler.

==> Extended Version/proof.tex <==
\section{Proof of Proposition \ref{main-body-mw}}
\label{bigproof}
Our proof follows the same procedure described over several chapters in \cite{neely} and is divided into two parts.

First, we consider a class of schedulers that make decisions based solely on the current bandwidth demands $\mathbf{W^e}(t)$ called $\mathbf{W^e}(t)$-only schedulers. Using \cite[Theorem 4.5]{neely}, we show that there exists a set of schedulers of this class that satisfies the premise of Proposition \ref{equiv2} for ergodic markovian demands.

Second, by following the steps in \cite[p.34-p.36]{neely}, we show that the Max-Weight scheduler strongly stabilizes the deficits $d_i(t)$ whenever that set of $\mathbf{W^e}(t)$-only schedulers stabilizes them. Thus, we show that the Max-Weight scheduler also satisfies the premise of Proposition \ref{equiv2} for ergodic markovian demands. 

The step-by-step details of the first part and the second part of this proof are in Appendix \ref{firstpart} and Appendix \ref{secondpart} respectively.

\subsection{$\mathbf{W^e(t)}$-only schedulers}
\label{firstpart}
Here, we show that there exists a set of $\mathbf{W^e}(t)$-only schedulers that satisfies the premise of Proposition \ref{equiv2} when $\mathbf{W}(t)$ follows an ergodic MC. Suppose $\mathbf{W}(t)$ follows an ergodic MC, and let $\pi_i^w$ denote the probability of state $w \in \mathcal{S}_i$, where $\mathcal{S}_i$ the state space of MC $i$. Since each MC $i$ is ergodic, it follows \cite[Corollary 9.29]{queuebook}:
\begin{equation}
 \liminf\limits_{T \to \infty}\frac{1}{T}\sum\limits_{t=1}^{T}\mathbbm{1}_{W_i(t) \leq W_i^r}=\sum_{w \in \mathcal{S}_i : w \leq W_i^r}\pi_i^w, \: w.p.1, \: \forall i.
\label{time-averages}
\end{equation}

From (\ref{time-averages}), it follows that assumption (\ref{assumption}) holds. Moreover, since the MC of $\mathbf{W}(t)$ is ergodic, its limiting distribution is the stationary distribution \cite[Theorem 9.4 and Theorem 8.6]{queuebook}. Therefore, regardless of the initial distribution of the MC, after some period of time, the process $\mathbf{W}(t)$ becomes identically distributed (id). 

Assuming that this transition period is small enough, we consider that the process once it has reached its stationary distribution. Thus, $\Pr(W_i(t)=w)=\pi_i^w, \,\forall t \in \mathbb{N}$, where $\pi_i$ is the stationary distribution of NS $i$ and $\pi_i^w$ is the probability of state $w$. Hence, the vector $\mathbf{W^e}(t)$ is also id with $\Pr(W_i^e(t)=w-W^L_i)=\pi_i^w, \, \forall w \in \mathcal{S}_i$. Let $\mathcal{S}_i^e \triangleq \{w^e: w^e+W^L_i \in \mathcal{S}_i\}$, $\mathcal{S}^e \triangleq \mathcal{S}_1^e \times ... \times \mathcal{S}_N^e$ and $p_i^{w^e} \triangleq \pi_i^{w^e+W^L_i}$, $\forall w^e \in \mathcal{S}_i^e$. Then, $\Pr(\mathbf{W^e}(t)=\mathbf{w^e})=\prod\limits_{i \leq N}p_i^{w^e_i} \triangleq p_{\mathbf{W^e}}(\mathbf{w^e})$, where $\mathbf{w^e} \in \mathcal{S}^e$.

Now, consider the class of $\mathbf{W^e}(t)$-only schedulers defined by probability distributions $p_{\mathbf{u}|\mathbf{w^e}}(\mathbf{u},\mathbf{w^e}) \triangleq \Pr(\mathbf{u}(t)=\mathbf{u}| \mathbf{W^e}(t)=\mathbf{w^e})$, i.e., if $\mathbf{W^e}(t)=\mathbf{w^e}$, then $\mathbf{u}(t)=\mathbf{u}$ with probability $p_{\mathbf{U}|\mathbf{W^e}}(\mathbf{u},\mathbf{w^e})$ which does not depend on time $t$. Note that $p_{\mathbf{U}|\mathbf{W^e}}(\mathbf{u},\mathbf{w^e})$ must satisfy:
\begin{equation}
\sum\limits_{\mathbf{u} \in \mathcal{U}(\mathbf{w^e},W^c)}p_{\mathbf{U}|\mathbf{W^e}}(\mathbf{u},\mathbf{w^e})=1, \: \forall \mathbf{w^e} \in \mathcal{S}^e.
\end{equation}
Next, we wish to compute the limit of the time average of $u_i(t)\mathbbm{1}_{W_i^e(t) > 0}$. To this end, first note that:
\begin{equation}
\begin{aligned}
& \E[u_i(t)\mathbbm{1}_{W_i^e(t) > 0}]= \bar{u_i} \triangleq\\
& \sum\limits_{\mathbf{w^e} \in \mathcal{S}^e, \mathbf{u} \in \mathcal{U}(\mathbf{w^e},W^c)}p_{\mathbf{U}|\mathbf{W^e}}(\mathbf{u},\mathbf{w^e})p_{\mathbf{W^e}}(\mathbf{w^e})u_i\mathbbm{1}_{W_i^e > 0}, \: \forall t.
\end{aligned}
\label{expectation}
\end{equation}
Since $u_i(t)\mathbbm{1}_{W_i^e(t) > 0}$ is modulated by the ergodic MC that $\{\mathbf{W^e}(t)\}_{t \in \mathbb{N}}$ follows, it holds \cite[p.76]{neely}:
\begin{equation}
\begin{aligned}
\liminf\limits_{T \to \infty}\frac{1}{T}\sum\limits_{t=1}^{T}u_i(t)\mathbbm{1}_{W_i^e(t) >0}=\frac{\E[\sum\limits_{t=1}^{T_1}u_i(t)\mathbbm{1}_{W_i^e(t) > 0}]}{\E[T_1]}, \: w.p.1,
\end{aligned}
\label{limit1}
\end{equation}
where $T_1$ is the first recurrence time to some arbitrary state $s \in \mathcal{S}^e$. Since $u_i(t)\mathbbm{1}_{W_i^e(t) > 0}$ is a bounded function of a finite-state and ergodic MC, the extension of Wald's equation for MCs in \cite{Moustakides} can be applied. Since we observe our MC after convergence to the stationary distribution, then the extension in \cite{Moustakides} results to the standard Wald's equation. Thus:
\begin{equation}
\liminf\limits_{T \to \infty}\frac{1}{T}\sum\limits_{t=1}^{T}u_i(t)\mathbbm{1}_{W_i^e(t) >0}=\bar{u_i}, \: w.p.1.
\label{limit2}
\end{equation}
Therefore, under an $\mathbf{W^e}(t)$-only scheduler, the long-term time-average of $u_i(t)\mathbbm{1}_{W_i^e(t) > 0}$ is equal to its one-slot expected value which is constant since $u_i(t)\mathbbm{1}_{W_i^e(t) > 0}$ is id. Now, consider the following constraints:
\begin{equation}
\begin{aligned}
& \liminf\limits_{T \to \infty}\frac{1}{T}\sum\limits_{t=1}^{T}\E[u_i(t)\mathbbm{1}_{W_i^e(t) >0}] \geq P_i^H - P_i^M,  \; \forall i,\\
& \mathbf{u}(t) \in \mathcal{U}(\mathbf{W^e}(t),W^c), \forall t.
\end{aligned}
\label{meanrate}
\end{equation}
Note that (\ref{meanrate}) is identical to the feasibility region of (\ref{schedprob4}) with the exception of the expected value operator $\E[\cdot]$ in the limit. Due to $(\ref{limit2})$, it can be shown that if there does not exist a $\mathbf{W^e}(t)$-only scheduler that satisfies (\ref{meanrate}), no scheduler satisfies (\ref{meanrate}) including non-causal schedulers \cite[Theorem 4.5]{neely}. 

Thus, Proposition \ref{equiv2} applies for a set of $\mathbf{W^e}(t)$-only schedulers, where $\mathcal{F}_{W^c}$ is defined by (\ref{meanrate}). Ideally, however we would like to show that it also applies for $\mathcal{F}_{W^c}=\mathcal{G}_{W^c}$. To this end, note that due to Fatou's lemma, it holds:
\begin{equation}
\begin{aligned}
& \liminf\limits_{T \to \infty}\frac{1}{T}\sum\limits_{t=1}^{T}u_i(t)\mathbbm{1}_{W_i^e(t) >0} \geq P_i^H - P_i^M, \: w.p.1 \\
\Rightarrow  & \liminf\limits_{T \to \infty}\frac{1}{T}\sum\limits_{t=1}^{T}\E[u_i(t)\mathbbm{1}_{W_i^e(t) >0}] \geq P_i^H - P_i^M, \: w.p.1.
\end{aligned}
\label{fatou}
\end{equation}
Using the above, we can show the following lemma.
\begin{lemma}
There exists $\mathcal{C'}\triangleq \{\mathbf{u}_{W^c}\}_{W^c \in \mathbb{R}}$ s.t. $\forall W^c \in \mathbb{R}$, if $\mathbf{u}_{W^c} \notin \mathcal{G}_{W^c}$, then $\mathcal{G}_{W^c}=\emptyset$, where each $\mathbf{u}_{W^c}$ is a $\mathbf{W^e}(t)$-only scheduler.

\noindent Proof:

We prove the contrapositive. Suppose $\exists \mathbf{v} \in \mathcal{G}_{W_c}$. Due to (\ref{fatou}), scheduler $\mathbf{v}$ satisfies (\ref{meanrate}). Thus, due to \cite[Theorem 4.5]{neely}, $\exists \mathbf{u}_{W^c}$ that satisfies (\ref{meanrate}) where $\mathbf{u}_{W^c}$ is a $\mathbf{W^e}(t)$-only scheduler. Thus, since (\ref{fatou}) holds with equivalence for $\mathbf{W^e}(t)$-only schedulers, $\mathbf{u}_{W^c} \in \mathcal{G}_{W_c}$ where $\mathbf{u}_{W^c}$ is $\mathbf{W^e}(t)$-only.

\label{adequacy}
\end{lemma}

Therefore, due to Proposition \ref{equiv2}, it is adequate to consider the set $\mathcal{C'}$ of $\mathbf{W^e}(t)$-only schedulers. Note that Lemma \ref{adequacy} shows the existence of set $\mathcal{C'}$ but it does not describe a method to find it. To find each $\mathbf{W^e(t)}$-only scheduler $\mathbf{u}_{W^c} \in \mathcal{C'}$, we need to solve the following problem for each $W^c \in \mathbb{R}$:
\begin{align}
& \underset{\epsilon_{W^c}, p_{\mathbf{U}|\mathbf{W^e}}}{\rm{maximize}} \qquad \epsilon_{W^c} \nonumber\\
& \text{s.t.:} \: \sum\limits_{\mathbf{u} \in \mathcal{U}(\mathbf{w^e},W^c)}p_{\mathbf{U}|\mathbf{W^e}}(\mathbf{u},\mathbf{w^e})=1, \: \forall \mathbf{w^e} \in \mathcal{S}^e, \nonumber \\
& \phantom{\text{s.t.:} \:} p_{\mathbf{U}|\mathbf{W^e}}(\mathbf{u},\mathbf{w^e}) \geq 0, \: \forall \mathbf{w^e} \in \mathcal{S}^e,\: \forall \mathbf{u} \in \mathcal{U}(\mathbf{w^e},W^c), \nonumber\\
& \phantom{\text{s.t.:} \:} \sum\limits_{\mathbf{w^e} \in \mathcal{S}^e, \mathbf{u} \in \mathcal{U}(\mathbf{w^e},W^c)}p_{\mathbf{U}|\mathbf{W^e}}(\mathbf{u},\mathbf{w^e})p_{\mathbf{W^e}}(\mathbf{w^e})u_i\mathbbm{1}_{W_i^e > 0} \nonumber \\
& \phantom{\text{s.t.:} \: \sum\limits_{\mathbf{w^e} \in \mathcal{S}^e, \mathbf{u} \in \mathcal{U}(\mathbf{w^e},W^c)}} \geq P_i^H - P_i^M + \epsilon_{W^c}, \: \forall i.
\label{findc}
\end{align}

In (\ref{findc}), the first two constraints ensure that the conditional distribution that defines the $\mathbf{W^e}(t)$-only scheduler is valid and the third constraint relates to the time-average constraint. Let $\epsilon^*_{W^c}$ denote the optimal value of (\ref{findc}). The optimal solutions of (\ref{findc}) for all $W^c \in \mathbb{R}$ compose set $\mathcal{C'}$. Clearly, if $\epsilon^*_{W^c}<0$, the long-term average constraint cannot be met by any $\mathbf{W^e}(t)$-only scheduler which means that no other scheduler can meet it as stated in Lemma \ref{adequacy}. Thus, if $\epsilon^*_{W^c}<0$, then $\mathcal{G}_{W^c} = \emptyset$.

\subsection{Max-Weight Scheduler}
\label{secondpart}
Our objective now is to show that the Max-Weight scheduler strongly stabilizes the deficits whenever $\epsilon^*_{W^c}<0$. If that is true, then it immediately follows from Lemma \ref{adequacy} and (\ref{rate-stability}) that the Max-Weight scheduler also satisfies the premise of Proposition \ref{equiv2} for ergodic markovian demands. To do so, we consider the following Lyapunov function:
\begin{equation}
L(\mathbf{d}(t)) \triangleq \frac{1}{2}\mathbf{1}^\top\mathbf{d}(t).
\label{lyapunov}
\end{equation}
Note that if $L(\mathbf{d}(t))$ is small then all deficits are small. Next, consider the conditional Lyapunov drift:
\begin{equation}
\Delta(\mathbf{d}(t)) \triangleq \E[L(\mathbf{d}(t+1))-L(\mathbf{d}(t))| \mathbf{d}(t)].
\label{drift}
\end{equation}
Note that if the conditional Lyapunov drift is small, then the deficits between two consecutive slots do not differ significantly. Following the same steps as in \cite[p.33]{neely}, we can show:
\begin{equation}
\begin{aligned}
\Delta(\mathbf{d}(t)) \leq  B + & \sum\limits_{i=1}^Nd_i(t)(P^H_i-P^M_i)\\
&-\E \left[\sum\limits_{i=1}^Nd_i(t)u_i(t)\mathbbm{1}_{W_i^e(t) > 0}|\mathbf{d}(t)\right],
\end{aligned}
\label{driftbound}
\end{equation}
where $B=1 + \sum_{i=1}^N(P^H_i-P^M_i)^2/N$. Note that since a small conditional drift implies "stable" deficits, we wish to reduce the conditional Lyapunov drift. To this end, we maximize the expectation in (\ref{driftbound}) by maximizing its argument. 

Thus, we need to derive a scheduler that observes the deficits $\mathbf{d}(t)$ and the bandwidth demands $\mathbf{W^e}(t)$, and maximizes the argument of the expectation in (\ref{driftbound}). This scheduler is precisely the Max-Weight scheduler defined in (\ref{max-weight}). Since the Max-Weight scheduler maximizes the expectation in (\ref{driftbound}), it holds:
\begin{equation}
\begin{aligned}
& \Delta(\mathbf{d}^*(t)) \leq B + \sum\limits_{i=1}^Nd_i^*(t)(P^H_i-P^M_i) \\
& -\E \left[\sum\limits_{i=1}^Nd^*_i(t)u_i(t)\mathbbm{1}_{W_i^e(t) > 0}|\mathbf{d}^*(t)\right], \: \forall \mathbf{u}(t) \in \mathcal{U}_{(\mathbf{w^e},W^c)},
\end{aligned}
\label{maxweightbound}
\end{equation}
where $\mathbf{d}^*(t)$ are the deficits under the Max-Weight scheduler. Since bound (\ref{maxweightbound}) holds for every possible scheduling decision $ \mathbf{u}(t) \in \mathcal{U}_{(\mathbf{w^e},W^c)}$, we can apply it for the $\mathbf{W^e}(t)$-only scheduler that solves (\ref{findc}). In that case, since $u_i(t)\mathbbm{1}_{W_i^e(t) > 0}$ is independent of deficits $\mathbf{d}^*(t)$ and  $\E[u_i(t)\mathbbm{1}_{W_i^e(t) > 0}]=P^H_i-P^M_i+\epsilon^*_{W^c}$, it holds:
\begin{equation}
\Delta(\mathbf{d}^*(t)) \leq B - \epsilon^*_{W^c}\sum\limits_{i=1}^Nd_i^*(t).
\label{newbound}
\end{equation}
By taking the expectation of (\ref{newbound}) and following the steps in \cite[p.36]{neely}, it holds:
\begin{equation}
\epsilon^*_{W^c}\limsup\limits_{T \to \infty}\frac{1}{T}\sum\limits_{t=1}^T\E[d^*_i(t)] \leq B, \: \forall i.
\label{almost-final}
\end{equation}

Therefore, if $\epsilon^*_{W^c}>0$, then all deficits $\mathbf{d}(t)$ are strongly stable. Due to (\ref{rate-stability}), it follows that the Max-Weight scheduler satisfies the time-average constraint whenever there exists a $\mathbf{W^e}(t)$-only scheduler that satisfies it. Let $\mathbf{u}'_{W^c}$ be the $\mathbf{W^e}(t)$-only scheduler defined by the solution of (\ref{findc}). Equivalently, if $\mathbf{u}'_{W^c} \in \mathcal{G}_{W^c}$, then $\mathbf{u}^*_{W^c} \in \mathcal{G}_{W^c}$. 

Given the above and Lemma \ref{adequacy}, it immediately follows that the Max-Weight scheduler satisfies the premise of Proposition \ref{equiv2} for $\mathcal{F}_{W^c}=\mathcal{G}_{W^c}$ when $\mathbf{W}(t)$ follows an ergodic MC. Therefore, our proof is finally complete.

